The seven-gluon amplitude in multi-Regge kinematics beyond leading logarithmic accuracy

We present an all-loop dispersion integral, well-defined to arbitrary logarithmic accuracy, describing the multi-Regge limit of the 2->5 amplitude in planar N=4 super Yang-Mills theory. It follows from factorization, dual conformal symmetry and consistency with soft limits, and specifically holds in the region where the energies of all produced particles have been analytically continued. After promoting the known symbol of the 2-loop N-particle MHV amplitude in this region to a function, we specialize to N=7, and extract from it the next-to-leading order (NLO) correction to the BFKL central emission vertex, namely the building block of the dispersion integral that had not yet appeared in the well-studied six-gluon case. As an application of our results, we explicitly compute the seven-gluon amplitude at next-to-leading logarithmic accuracy through 5 loops for the MHV case, and through 3 and 4 loops for the two independent NMHV helicity configurations, respectively.

==> ghTexMHV.tex <==
\begin{align}
\tilde{g}_{+++}^{(2;0,0)} \left( \rho_1, \rho_2 \right) = &\frac{1}{4}\cG_{0,0,1}\left(\rho_1\right)+\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)-\frac{1}{4}\cG_{0,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_{0,1,1}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,1}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{0,\rho_2,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_{1,0,0}\left(\rho_1\right)+\frac{1}{4}\cG_{1,0,0}\left(\rho_2\right)-\frac{1}{4}\cG_{1,0,1}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_{1,0,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_{1,1,0}\left(\rho_2\right)+\frac{1}{2}\cG_{1,1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{2}\cG_{1,1,1}\left(\rho_2\right)-\frac{1}{8}\cG_{1,\rho_2,0}\left(\rho_1\right)+\frac{1}{4}\cG_{1,\rho_2,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2,1,0}\left(\rho_1\right)-\frac{1}{4}\zeta_2\cG_0\left(\rho_1\right)+\frac{1}{4}\zeta_2\cG_1\left(\rho_1\right)+\frac{1}{4}\zeta_2\cG_1\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\tilde{h}_{+++}^{(2;0,0)} \left( \rho_1, \rho_2 \right) = &\frac{1}{16}\cG_{0,0}\left(\rho_1\right)-\frac{1}{16}\cG_{0,1}\left(\rho_1\right)-\frac{1}{16}\cG_{1,0}\left(\rho_1\right)+\frac{1}{16}\cG_{1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{16}\cG_{1,1}\left(\rho_2\right)-\frac{1}{16}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)+\frac{1}{16}\cG_1\left(\rho_1\right)\cG_1\left(\rho_2\right)
\end{align}
%
%
%\begin{align}
%\tilde{g}_{+++}^{(3;1,0)} \left( \rho_1, \rho_2 \right) = &\frac{3}{16}\cG_{0,0,0,1}\left(\rho_1\right)-\frac{1}{16}\cG_{0,0,1,0}\left(\rho_1\right)-\frac{3}{8}\cG_{0,0,1,1}\left(\rho_1\right)+\frac{1}{16}\cG_{0,0,1,\rho_2}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_{0,0,\rho_2,1}\left(\rho_1\right)-\frac{1}{16}\cG_{0,1,0,0}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,0,1}\left(\rho_1\right)+\frac{3}{4}\cG_{0,1,1,1}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_{0,1,\rho_2,\rho_2}\left(\rho_1\right)+\frac{1}{16}\cG_{0,\rho_2,0,1}\left(\rho_1\right)+\frac{1}{4}\cG_{0,\rho_2,1,1}\left(\rho_1\right)-\frac{1}{8}\cG_{0,\rho_2,1,\rho_2}\left(\rho_1\right)\\
% \nonumber &+\frac{3}{16}\cG_{1,0,0,0}\left(\rho_1\right)-\frac{1}{2}\cG_{1,0,0,1}\left(\rho_1\right)-\frac{1}{16}\cG_{1,0,0,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,1,0}\left(\rho_1\right)\\
% \nonumber &+\frac{3}{4}\cG_{1,0,1,1}\left(\rho_1\right)+\frac{1}{16}\cG_{1,0,1,\rho_2}\left(\rho_1\right)+\frac{1}{16}\cG_{1,0,\rho_2,0}\left(\rho_1\right)+\frac{1}{16}\cG_{1,0,\rho_2,1}\left(\rho_1\right)\\
% \nonumber &-\frac{3}{8}\cG_{1,1,0,0}\left(\rho_1\right)+\frac{3}{4}\cG_{1,1,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,1,0,\rho_2}\left(\rho_1\right)+\frac{3}{4}\cG_{1,1,1,0}\left(\rho_1\right)\\
% \nonumber &-\frac{3}{2}\cG_{1,1,1,1}\left(\rho_1\right)-\frac{3}{16}\cG_{1,1,1,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_{1,1,\rho_2,0}\left(\rho_1\right)-\frac{5}{16}\cG_{1,1,\rho_2,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{8}\cG_{1,1,\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{16}\cG_{1,\rho_2,0,0}\left(\rho_1\right)+\frac{1}{16}\cG_{1,\rho_2,0,1}\left(\rho_1\right)+\frac{1}{16}\cG_{1,\rho_2,0,\rho_2}\left(\rho_1\right)\\
% \nonumber &-\frac{5}{16}\cG_{1,\rho_2,1,1}\left(\rho_1\right)+\frac{1}{16}\cG_{1,\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{16}\cG_{\rho_2,0,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,0,1,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_{\rho_2,0,1,\rho_2}\left(\rho_1\right)+\frac{1}{16}\cG_{\rho_2,0,\rho_2,1}\left(\rho_1\right)+\frac{1}{16}\cG_{\rho_2,1,0,0}\left(\rho_1\right)+\frac{1}{16}\cG_{\rho_2,1,0,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_{\rho_2,1,0,\rho_2}\left(\rho_1\right)-\frac{3}{16}\cG_{\rho_2,1,1,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,1,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1,\rho_2,0}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{16}\cG_{\rho_2,1,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,\rho_2,1,0}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,\rho_2,1,1}\left(\rho_1\right)+\frac{1}{2}\zeta_2\cG_{0,1}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{2}\zeta_2\cG_{1,0}\left(\rho_1\right)-\zeta_2\cG_{1,1}\left(\rho_1\right)-\frac{1}{2}\zeta_3\cG_1\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_{0,0}\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)+\frac{1}{16}\cG_{0,1}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)-\frac{3}{16}\cG_{0,1}\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_{0,0}\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{1}{16}\cG_{0,1}\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{3}{16}\cG_{0,1}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)\\
% \nonumber &+\frac{1}{16}\cG_{0,\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{3}{16}\cG_{1,0}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{4}\cG_{0,0}\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)\\
% \nonumber &+\frac{3}{16}\cG_{0,1}\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)+\frac{3}{16}\cG_{1,0}\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)+\frac{1}{4}\cG_{0,\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
% \nonumber &+\frac{1}{8}\cG_{1,0}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{1}{8}\cG_{1,1}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{3}{16}\cG_{0,0}\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
% \nonumber &+\frac{3}{16}\cG_{0,1}\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0}\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,1}\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_{0,1}\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)+\frac{1}{16}\cG_{1,0}\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)+\frac{1}{8}\cG_{1,1}\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{16}\cG_{0,0}\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1}\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)-\frac{1}{16}\cG_{1,0}\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_{0,1}\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{1,1}\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)-\frac{3}{16}\cG_1\left(\rho_1\right)\cG_{0,0,0}\left(\rho_2\right)\\
% \nonumber &+\frac{1}{16}\cG_0\left(\rho_2\right)\cG_{0,0,1}\left(\rho_1\right)-\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{0,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,0,1}\left(\rho_2\right)\\
% \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,0,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{0,1,0}\left(\rho_2\right)-\frac{1}{16}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1,0}\left(\rho_2\right)\\
% \nonumber &+\frac{1}{16}\cG_1\left(\rho_1\right)\cG_{0,1,1}\left(\rho_2\right)-\frac{3}{16}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1,1}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,1,\rho_2}\left(\rho_1\right)
% \end{align}
% %
% %
% \begin{align}
% \nonumber &-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,\rho_2,0}\left(\rho_1\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,\rho_2,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,\rho_2,1}\left(\rho_1\right)-\frac{1}{16}\cG_0\left(\rho_2\right)\cG_{1,0,0}\left(\rho_1\right)+\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{1,0,0}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{1,0,0}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,0,1}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_1\left(\rho_1\right)\cG_{1,0,1}\left(\rho_2\right)-\frac{1}{16}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0,1}\left(\rho_2\right)-\frac{1}{16}\cG_0\left(\rho_2\right)\cG_{1,0,\rho_2}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{1,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,1,0}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{16}\cG_1\left(\rho_1\right)\cG_{1,1,0}\left(\rho_2\right)+\frac{1}{16}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1,0}\left(\rho_2\right)-\frac{3}{16}\cG_0\left(\rho_2\right)\cG_{1,1,1}\left(\rho_1\right)\\
% \nonumber &+\frac{3}{16}\cG_1\left(\rho_2\right)\cG_{1,1,1}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{1,1,1}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1,1}\left(\rho_2\right)\\
% \nonumber &-\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{1,1,\rho_2}\left(\rho_1\right)+\frac{7}{16}\cG_1\left(\rho_2\right)\cG_{1,1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,\rho_2,0}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,\rho_2,0}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,\rho_2,1}\left(\rho_1\right)-\frac{1}{16}\cG_0\left(\rho_2\right)\cG_{\rho_2,0,1}\left(\rho_1\right)\\
% \nonumber &-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,1,0}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,1,1}\left(\rho_1\right)+\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{\rho_2,1,1}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{16}\cG_0\left(\rho_2\right)\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2,0}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2,1}\left(\rho_1\right)
%\end{align}
%%
%%
%\begin{align}
%\tilde{h}_{+++}^{(3;1,0)} \left( \rho_1, \rho_2 \right) = &-\frac{1}{16}\cG_{0,0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1,0}\left(\rho_1\right)+\frac{1}{8}\cG_{0,1,1}\left(\rho_1\right)-\frac{1}{16}\cG_{1,0,0}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{8}\cG_{1,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,1,0}\left(\rho_1\right)-\frac{1}{8}\cG_{1,1,1}\left(\rho_1\right)\\
% \nonumber &+\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)+\frac{1}{16}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)
%\end{align}
%
%


==> ghTexNMHV.tex <==
\beq\bsp
\tilde{g}_{-++}^{(2;0,0)} \left(\rho_1,\rho_2\right) = &\mathfrak{ga}^{\text{(2;0,0)}}_{-++}\left(\rho_1,\rho_2\right)+R_{234}\mathfrak{gb}_{1,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)+R_{235}\mathfrak{gb}_{2,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)
\esp\eeq
%
%
\begin{align}
\mathfrak{ga}^{\text{(2;0,0)}}_{-++}\left(\rho_1,\rho_2\right) = &\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,0}\left(\rho_2\right)-\frac{1}{4}\cG_{0,1,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_{1,0,0}\left(\rho_1\right)+\frac{1}{4}\cG_{1,0,0}\left(\rho_2\right)-\frac{1}{4}\cG_{1,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{1,0,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{4}\cG_{1,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_{1,1,0}\left(\rho_2\right)+\frac{1}{2}\cG_{1,1,1}\left(\rho_2\right)-\frac{1}{4}\cG_{1,1,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{1,\rho_2,0}\left(\rho_1\right)-\frac{1}{4}\cG_{1,\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{\rho_2,0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{4}\cG_{\rho_2,1,1}\left(\rho_1\right)+\frac{1}{4}\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{4}\zeta_2\cG_0\left(\rho_1\right)-\frac{1}{4}\zeta_2\cG_1\left(\rho_1\right)+\frac{1}{4}\zeta_2\cG_1\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)+\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)+\frac{1}{2}\cG_1\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{4}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)-\frac{1}{2}\cG_1\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{gb}_{1,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &-\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1,0}\left(\rho_2\right)-\frac{1}{4}\cG_{0,1,1}\left(\rho_1\right)+\frac{3}{8}\cG_{0,1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{0,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{0,\rho_2,1}\left(\rho_1\right)-\frac{1}{8}\cG_{1,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_{1,1,0}\left(\rho_2\right)-\frac{1}{4}\cG_{1,1,1}\left(\rho_2\right)+\frac{1}{8}\cG_{1,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_{\rho_2,1,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_0\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{4}\cG_0\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{gb}_{2,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{3}{8}\cG_{0,0,0}\left(\rho_1\right)-\frac{3}{8}\cG_{0,0,0}\left(\rho_2\right)+\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{0,0,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{4}\cG_{0,1,0}\left(\rho_1\right)+\frac{3}{8}\cG_{0,1,0}\left(\rho_2\right)+\frac{1}{4}\cG_{0,1,1}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_{0,\rho_2,0}\left(\rho_1\right)+\frac{1}{4}\cG_{0,\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,0}\left(\rho_1\right)+\frac{1}{4}\cG_{1,0,0}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{1,0,1}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{1,0,\rho_2}\left(\rho_1\right)+\frac{1}{2}\cG_{1,1,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2,0,0}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,0,\rho_2}\left(\rho_1\right)+\frac{1}{2}\zeta_2\cG_0\left(\rho_1\right)-\zeta_3\\
 \nonumber &-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,0}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,0}\left(\rho_1\right)+\frac{1}{4}\cG_0\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{4}\cG_0\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{1}{4}\cG_0\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)+\frac{1}{2}\cG_0\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)
\end{align}
%
%
\beq\bsp
\tilde{h}_{-++}^{(2;0,0)} \left(\rho_1,\rho_2\right) = &\mathfrak{ha}^{\text{(2;0,0)}}_{-++}\left(\rho_1,\rho_2\right)+R_{234}\mathfrak{hb}_{1,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)+R_{235}\mathfrak{hb}_{2,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)
\esp\eeq
%
%
\begin{align}
\mathfrak{ha}^{\text{(2;0,0)}}_{-++}\left(\rho_1,\rho_2\right) = &\frac{1}{16}\cG_{0,0}\left(\rho_1\right)+\frac{1}{16}\cG_{0,1}\left(\rho_1\right)-\frac{1}{16}\cG_{1,0}\left(\rho_1\right)+\frac{1}{16}\cG_{1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{16}\cG_{1,1}\left(\rho_2\right)-\frac{1}{16}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)-\frac{1}{16}\cG_1\left(\rho_1\right)\cG_1\left(\rho_2\right)
\end{align}
%
%
\begin{align}
\mathfrak{hb}_{1,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &0
\end{align}
%
%
\begin{align}
\mathfrak{hb}_{2,-++}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &-\frac{1}{8}\cG_{0,0}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)
\end{align}
%
%
\beq\bsp
\tilde{g}_{-+-}^{(2;0,0)} \left(\rho_1,\rho_2\right) &= \, \mathfrak{ga}^{\text{(2;0,0)}}_{-+-}\left(\rho_1,\rho_2\right)+R_{234}\mathfrak{gb}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) \\
&+\bar{R}_{345}\mathfrak{gb}_{2,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)+R_{234}\bar{R}_{345}\mathfrak{gc}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)
\esp\eeq
%
%
\begin{align}
\mathfrak{ga}^{\text{(2;0,0)}}_{-+-}\left(\rho_1,\rho_2\right) = &-\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1,0}\left(\rho_2\right)-\frac{1}{8}\cG_{0,1,1}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{0,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,1,0}\left(\rho_1\right)+\frac{5}{8}\cG_{1,1,1}\left(\rho_1\right)\\
 \nonumber &-\frac{3}{8}\cG_{1,\rho_2,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1,0}\left(\rho_1\right)-\frac{1}{2}\cG_{\rho_2,1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_{\rho_2,\rho_2,1}\left(\rho_1\right)-\frac{1}{4}\zeta_2\cG_0\left(\rho_1\right)+\frac{1}{4}\zeta_2\cG_1\left(\rho_1\right)-\frac{1}{4}\zeta_2\cG_1\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{5}{8}\cG_1\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{1}{4}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)+\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)+\frac{1}{2}\cG_1\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{gb}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{1}{4}\cG_{0,0,1}\left(\rho_1\right)+\frac{3}{4}\cG_{0,0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{0,1,0}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{2}\cG_{0,1,1}\left(\rho_1\right)-\frac{1}{2}\cG_{0,1,1}\left(\rho_2\right)-\frac{1}{8}\cG_{0,\rho_2,1}\left(\rho_1\right)-\frac{3}{8}\cG_{1,0,1}\left(\rho_1\right)\\
 \nonumber &-\frac{3}{8}\cG_{1,0,1}\left(\rho_2\right)+\frac{5}{8}\cG_{1,1,1}\left(\rho_2\right)+\frac{3}{8}\cG_{1,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2,1,0}\left(\rho_1\right)+\frac{1}{2}\cG_{\rho_2,1,1}\left(\rho_1\right)-\frac{1}{4}\cG_{\rho_2,\rho_2,1}\left(\rho_1\right)+\frac{1}{2}\zeta_2\cG_1\left(\rho_2\right)\\
 \nonumber &+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{0,0}\left(\rho_1\right)-\frac{3}{8}\cG_0\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{2}\cG_1\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{3}{8}\cG_1\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{4}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{2}\cG_1\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{gb}_{2,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{3}{8}\cG_{0,0,0}\left(\rho_2\right)-\frac{1}{4}\cG_{0,0,1}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1,0}\left(\rho_1\right)-\frac{1}{4}\cG_{0,1,0}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{0,1,1}\left(\rho_1\right)+\frac{1}{2}\cG_{0,1,1}\left(\rho_2\right)-\frac{1}{8}\cG_{0,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{0,\rho_2,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_{0,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{0,\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,0}\left(\rho_1\right)-\frac{1}{8}\cG_{1,0,1}\left(\rho_1\right)\\
 \nonumber &-\frac{3}{8}\cG_{1,1,0}\left(\rho_1\right)-\frac{5}{8}\cG_{1,1,1}\left(\rho_1\right)+\frac{1}{4}\cG_{1,1,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_{1,\rho_2,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_{1,\rho_2,1}\left(\rho_1\right)-\frac{3}{8}\cG_{1,\rho_2,\rho_2}\left(\rho_1\right)+\frac{1}{4}\cG_{\rho_2,0,0}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_{\rho_2,1,0}\left(\rho_1\right)+\frac{1}{2}\cG_{\rho_2,1,1}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,\rho_2,0}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_{\rho_2,\rho_2,1}\left(\rho_1\right)+\frac{1}{4}\cG_{\rho_2,\rho_2,\rho_2}\left(\rho_1\right)+\frac{1}{2}\zeta_2\cG_0\left(\rho_2\right)-\frac{1}{2}\zeta_2\cG_1\left(\rho_1\right)\\
 \nonumber &+\frac{1}{2}\zeta_2\cG_{\rho_2}\left(\rho_1\right)-\frac{\zeta_3}{2}+\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)+\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)-\frac{1}{2}\cG_1\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{2}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{3}{8}\cG_0\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)-\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{gc}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{3}{8}\cG_{0,0,0}\left(\rho_1\right)-\frac{9}{8}\cG_{0,0,0}\left(\rho_2\right)-\frac{1}{4}\cG_{0,0,1}\left(\rho_1\right)+\frac{5}{8}\cG_{0,0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{3}{8}\cG_{0,0,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1,0}\left(\rho_1\right)+\frac{7}{8}\cG_{0,1,0}\left(\rho_2\right)+\frac{1}{2}\cG_{0,1,1}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{2}\cG_{0,1,1}\left(\rho_2\right)+\frac{3}{8}\cG_{0,1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_{0,\rho_2,0}\left(\rho_1\right)+\frac{1}{4}\cG_{0,\rho_2,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{0,\rho_2,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,0,0}\left(\rho_1\right)+\frac{5}{8}\cG_{1,0,0}\left(\rho_2\right)+\frac{3}{8}\cG_{1,0,1}\left(\rho_1\right)\\
 \nonumber &-\frac{3}{8}\cG_{1,0,1}\left(\rho_2\right)+\frac{3}{8}\cG_{1,0,\rho_2}\left(\rho_1\right)+\frac{1}{2}\cG_{1,1,0}\left(\rho_1\right)-\frac{1}{2}\cG_{1,1,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{2}\cG_{1,1,\rho_2}\left(\rho_1\right)-\frac{1}{4}\cG_{1,\rho_2,0}\left(\rho_1\right)-\frac{3}{8}\cG_{1,\rho_2,1}\left(\rho_1\right)+\frac{1}{8}\cG_{1,\rho_2,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_{\rho_2,0,0}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,0,1}\left(\rho_1\right)-\frac{3}{8}\cG_{\rho_2,1,0}\left(\rho_1\right)-\frac{1}{2}\cG_{\rho_2,1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2,1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,\rho_2,0}\left(\rho_1\right)+\frac{1}{8}\cG_{\rho_2,\rho_2,1}\left(\rho_1\right)-\frac{1}{4}\cG_{\rho_2,\rho_2,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{2}\zeta_2\cG_0\left(\rho_1\right)-\frac{1}{2}\zeta_2\cG_0\left(\rho_2\right)-\frac{1}{2}\zeta_2\cG_{\rho_2}\left(\rho_1\right)-\frac{\zeta_3}{2}\\
 \nonumber &-\frac{3}{8}\cG_0\left(\rho_2\right)\cG_{0,0}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{0,0}\left(\rho_1\right)+\frac{5}{8}\cG_0\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{2}\cG_1\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)-\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,0}\left(\rho_2\right)+\frac{3}{8}\cG_0\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)\\
 \nonumber &-\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{0,1}\left(\rho_1\right)-\frac{3}{8}\cG_0\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{4}\cG_1\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{0,1}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)-\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{0,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{3}{8}\cG_0\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,0}\left(\rho_1\right)-\frac{1}{2}\cG_0\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)\\
 \nonumber &+\frac{3}{8}\cG_1\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)+\frac{1}{8}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,0}\left(\rho_2\right)-\frac{1}{2}\cG_0\left(\rho_2\right)\cG_{1,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{2}\cG_0\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)-\frac{1}{2}\cG_{\rho_2}\left(\rho_1\right)\cG_{1,1}\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{4}\cG_1\left(\rho_2\right)\cG_{1,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,0}\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)\\
 \nonumber &+\frac{3}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,1}\left(\rho_1\right)-\frac{1}{4}\cG_0\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2,\rho_2}\left(\rho_1\right)
\end{align}
%
%
\beq\bsp
\tilde{h}_{-+-}^{(2;0,0)} \left(\rho_1,\rho_2\right) &= \, \mathfrak{ha}^{\text{(2;0,0)}}_{-+-}\left(\rho_1,\rho_2\right)+R_{234}\mathfrak{hb}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) \\
&+\bar{R}_{345}\mathfrak{hb}_{2,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)+R_{234}\bar{R}_{345}\mathfrak{hc}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right)
\esp\eeq
%
%
\begin{align}
\mathfrak{ha}^{\text{(2;0,0)}}_{-+-}\left(\rho_1,\rho_2\right) = &\frac{1}{16}\cG_{0,0}\left(\rho_1\right)-\frac{1}{16}\cG_{0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1}\left(\rho_2\right)-\frac{1}{16}\cG_{1,0}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{16}\cG_{1,1}\left(\rho_1\right)+\frac{1}{16}\cG_{1,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{16}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)-\frac{1}{16}\cG_1\left(\rho_1\right)\cG_1\left(\rho_2\right)
\end{align}
%
%
\begin{align}
\mathfrak{hb}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{1}{8}\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)+\frac{1}{8}\cG_1\left(\rho_1\right)\cG_1\left(\rho_2\right)
\end{align}
%
%
\begin{align}
\mathfrak{hb}_{2,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &\frac{1}{8}\cG_{0,0}\left(\rho_2\right)+\frac{1}{8}\cG_{0,1}\left(\rho_1\right)+\frac{1}{8}\cG_{0,1}\left(\rho_2\right)-\frac{1}{8}\cG_{0,\rho_2}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_{1,0}\left(\rho_2\right)+\frac{1}{8}\cG_{1,\rho_2}\left(\rho_1\right)-\frac{1}{8}\cG_{\rho_2,1}\left(\rho_1\right)\\
 \nonumber &-\frac{1}{8}\cG_0\left(\rho_1\right)\cG_0\left(\rho_2\right)+\frac{1}{8}\cG_0\left(\rho_2\right)\cG_1\left(\rho_1\right)-\frac{1}{8}\cG_1\left(\rho_1\right)\cG_1\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2}\left(\rho_1\right)
\end{align}
%
%
\begin{align}
\mathfrak{hc}_{1,-+-}^{\text{(2;0,0)}}\left(\rho_1,\rho_2\right) = &-\frac{1}{8}\cG_{0,0}\left(\rho_1\right)-\frac{1}{8}\cG_{0,0}\left(\rho_2\right)-\frac{1}{8}\cG_{0,1}\left(\rho_1\right)-\frac{1}{8}\cG_{0,1}\left(\rho_2\right)\\
 \nonumber &+\frac{1}{8}\cG_{0,\rho_2}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0}\left(\rho_1\right)+\frac{1}{8}\cG_{1,0}\left(\rho_2\right)-\frac{1}{8}\cG_{1,\rho_2}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_{\rho_2,1}\left(\rho_1\right)\\
 \nonumber &+\frac{1}{8}\cG_0\left(\rho_1\right)\cG_0\left(\rho_2\right)-\frac{1}{8}\cG_0\left(\rho_2\right)\cG_1\left(\rho_1\right)+\frac{1}{8}\cG_0\left(\rho_1\right)\cG_1\left(\rho_2\right)\\
 \nonumber &-\frac{1}{8}\cG_1\left(\rho_2\right)\cG_{\rho_2}\left(\rho_1\right)
\end{align}
%
%

